DroidWalker: Generating Reproducible Test Cases via Automatic Exploration of Android Apps

Generating test cases through automatic app exploration is very useful for analyzing and testing Android apps. However, test cases generated by current app-exploration tools are not reproducible, i.e. when the generated test case is re-executed, the app cannot reach the same state as the explored one. As a result, app developers are not able to reproduce the failure or crash reported during the exploration, to conduct regression test after fixing the bug, or to execute the same test in different environments. In this paper, we present DroidWalker, a dynamic-analysis tool to generate reproducible test cases for Android apps. The key design of our tool is a dynamic-adaptive model that can abstract the app state in a proper granularity so every state in the model can be reached afterwards. Given an app under test, DroidWalker first explores the app to build the model. Then developers can select the state in the model to be reproduced. Finally, DroidWalker executes all the generated test cases and the app could reach exactly the same state as the explored one. We apply DroidWalker in three real usage scenarios to demonstrate its practical usage. The video of our tool is at https://youtu.be/ndUD8Gxs800.

==> section/_region_.tex <==
\message{ !name(Usage_scenarios.tex)}
\message{ !name(Usage_scenarios.tex) !offset(-2) }
\begin{figure}[t!]
\centering
  \includegraphics[width=0.45\textwidth]{./picture/test}
  \caption{Boxplot of the line coverage result across 20 benchmark apps.}~\label{fig:res}
\end{figure}

\begin{table*}[t!]
\scriptsize
\caption{Activity and method coverage result across five commercial app experiment, comparing with Monkey.}
\label{tab:seven_table}
\centering
\begin{tabular}[t]{|c|c|c|c|c|c|c|}
    \hline
    \textbf{App} & \textbf{Category} & \textbf{\tabincell{c}{Total\\ Activities}} & \textbf{\tabincell{c}{Activity Coverage\\ of DroidWalker}} & \textbf{\tabincell{c}{Activity Coverage\\ of Monkey}} & \textbf{\tabincell{c}{Method Coverage\\ of DroidWalker}} & \textbf{\tabincell{c}{Method Coverage\\ of Monkey}} \\ \hline
    \textbf{accuweather} & weather  &    37    &    11    &   8   &   2314     &     1786 \\
    \hline
    \textbf{lionbattery} & tools    &    100   &    29    &   23  &   2034     &     1317 \\
    \hline
    \textbf{iconology} & comics     &    41    &    22    &   18  &   3039     &     2253 \\
    \hline
    \textbf{fibit} & Health         &    92    &    28    &   21  &   6702     &     4927 \\
    \hline
    \textbf{vyapar} & Business      &    88    &    39    &   36   &  2543     &     1759\\
    \hline
\end{tabular}
\end{table*}

DroidWalker is designed to automatically generate reproducible test cases for Android apps. The current implementation offers a command-line tool and a visualized webpage. This section demonstrates three main usage scenarios of DroidWalker: (1) automate app exploration, (2) customize detection functions (3) reproduce target state.

\subsection{Automate App Exploration}

The first usage scenario is using DroidWalker to explore app under test automatically. Users should follow steps below:
\begin{enumerate}
\item Prepare the apk of the app to be explored. Then run a python script to repackage and build the app. The script can be configured with command-line arguments below, the repackaged project is located in the <lists> folder under the working directory:

\begin{tiny}
\begin{lstlisting}[ language=C]
python buildAndResigned.py APK\_Address
[--ip<address>] [--port<port>] [--output<graph|report|both>]
\end{lstlisting}
\end{tiny}


* [--ip<address> --port<port>]: optional, specify ip and port of the server used to upload exploring output, default to be localhost:5000
* [--output<graph|report|both>]:  optional, specify whether to output coverage report and the content of output, including a graph which is a visualization of the constructed GUI model, a progressive coverage plot over time. The default argument is both.

The output information will be visualized on the webpage. If the source code of the app under test is available, users can choose to instrument the app with Emma to get a more detailed coverage report or the coverage information will be generated using logcat and tracedump offered by Android SDK.

\item Start the server of visualized webpage using the command line: \emph{python server.py}, the console will output the specific listening port of the server.


\item Open Android emulator or connect with Android devices, then change directory to <lists/TestAPP/app/build/outputs/apk>. Start exploring the app using the command line: \emph{./runTest.sh}



\item Open a browser and enter the listening address of the server, and start monitoring the exploring output.
The webpage consists of a tab panel. By clicking the tab, user can switch between graph and coverage report. The webpage also demonstrates snapshots of the app, each of which corresponds to a specific node in the graph.

\end{enumerate}

To assess the efficiency of DroidWalker when applied to automate app exploration, we conduct two experiments to address the following two questions: first, whether our tool is superior than other automated exploring tools on a standard benchmark. Second, whether the tool can be applied to highly complex commercial apps.

For the first question, in order to be comparable, we use a set of mobile app benchmarks collected in the work done by Choudhary \textit{et al.}~\cite{Choudhary2016Automated}, and concerned both the code coverage and the coverage time as criteria to evaluate our tool.

The experiment setup is as follows:


1) Experiment 1: We ran our tool in the same setting as Choudhary \textit{et al.}~\cite{Choudhary2016Automated}, using the Ubuntu virtual machine configured with 2 cores and 6GB RAM, and an android emulator was configured with 4GB RAM. Each tool was allowed to run for 1 hour on each benchmark app. We chose Android SDK version 18 (Jelly Bean) to evaluate our tool based on the compatibility of most benchmark apps. To avoid unexpected side effects between tools and app, the emulator is destroyed after finishing each run. We repeated exploring each app for 3 times. From Fig.~\ref{fig:res}, we can see that line coverage of our tool is higher than those of the state-of-art tools, especially the model-based tools, such as A3E,GUIRipper and PUMA.

Although exploring a common set of apps is necessary for comparison, the fact that most apps in benchmarks are small and has simple logics indicates the result could not represent the performance of exploring tool on modern commercial apps. Thus, we select ten top apps from different categories on the Google Play and use the same two criteria to evaluate those apps. The experiment setup is as follows:

2) Experiment 2: Five top apps in Google Play are chosen to be tested. Because the applicaitons are more complicated, we chose Genymotion, an optimized android emulator to perform the experiment. The emulator settings are identical to Experiment 1. From Table~\ref{tab:seven_table}, we can see that our tool outperforms monkey even on complex commercial apps.




\subsection{Customize Detection Function}

The second usage scenario is using DroidWalker to customize detection function which can be called during exploration. User can write their own class under <config> directory. The class should be inherited from \texttt{Customize} class and override three methods--input, output and operate. Add the following argument while repackaging and building the app:
$*[--configure-class <Customized\_class>]$

The Customize class contains an outputContent field. The input method is designed to accept existing data in string format provided by users. The operate method is designed to be the central customized detection function. The output method is designed to deal with output, which is default to be sent to the server of visualized webpage.

Customized class will be instantiated inside the testing program and called during exploration. User can customize their own class to detect advertisements, code defects or code vulnerability. To demostrate customizing testing function, we write an exception collection class as example. The configuration of Android emulator is the same as experiment 2. The class example is as follows:

\begin{tiny}
\begin{lstlisting}[language=java, label = {code:except}]
public class ExceptionCollector extends Customize {
  public void operate(){
    Process process = Runtime.getRuntime().exec("logcat -d PACKAGE_NAME:I");
    BufferedReader bufferedReader = new BufferedReader(
        new InputStreamReader(process.getInputStream()));
    StringBuilder log = new StringBuilder();
    String line = "";
    Boolean flag = false, has_except = false;
    while ((line = bufferedReader.readLine()) != null) {
      if (line.contains("Exception")){
        flag = has_except = true;
        log.append(line + "\n");
      }else if(flag){
        if (line.contains("at")) log.append(line + "\n");
        else flag = false;
      }
    }
    Runtime.getRuntime().exec("logcat -c");
    if (has_except) outputContent = log.toString();
  }
}
\end{lstlisting}
\end{tiny}

then repackage and build the project using:

\begin{tiny}
\begin{lstlisting}[language=python]
python buildAndResigned.py APK --configure-class ExceptionCollector
\end{lstlisting}
\end{tiny}


We applied our tool to Fitbit, a top health care appliaction on Google Play. The tool recorded two exceptions during exploration. The first one is java.lang.UnsupportedOperationException, which suggests the testing program attempted to open a session that has a pending request to the user's FaceBook account. The second one is java.io.FileNotFoundException, which was raised when the testing program attempted to take pictures or select photo from album for profile. The trace information is as follows:


\begin{tiny}
\begin{lstlisting}[language=python]
failed to get https://android-api.fitbit.com/1/user/5NZZKF/badges.json
from cache  java.io.FileNotFoundException:
/data/data/com.fitbit.FitbitMobile/cache/datacache/https%3A%2F%2Fandroid
-api.fitbit.com%2F1%2Fuser%2F5NZZKF%2Fbadges.json:
 open failed: ENOENT (No such file or directory)
    at libcore.io.IoBridge.open(IoBridge.java:409)
    at java.io.FileInputStream.<init>(FileInputStream.java:78)
    at com.fitbit.data.repo.q.a(SourceFile:71)
    at com.fitbit.serverinteraction.ServerGateway.b(SourceFile:811)
    at com.fitbit.serverinteraction.ServerGateway.a(SourceFile:780)
    at com.fitbit.serverinteraction.PublicAPI.a(SourceFile:352)
    at com.fitbit.serverinteraction.PublicAPI.b(SourceFile:2376)
    at com.fitbit.data.bl.BadgesBusinessLogic.a(SourceFile:171)
    at com.fitbit.profile.ui.badges.a.c(SourceFile:48)
    at com.fitbit.profile.ui.badges.a.b_(SourceFile:18)
    at com.fitbit.util.bd.loadInBackground(SourceFile:36)
     ...
\end{lstlisting}
\end{tiny}

\subsection{Reproduce Target State}
The third usage is using DroidWalker to reproduce target states. DroidWalker will number each UI status. User can relate UI number with its corresponding snapshot and customize UI number sequence. The app uses Breath-First-Search strategy to generate a sequence of test cases, which are sorted by their event length, and these test cases will be executed one by one.

Users can detect severe code errors when DroidWalker encounters a crash. After revising related code, user can enter the UI number causing the crash to check whether the error has been fixed. Users can also make use of the customized detection functions, repeating test cases and checking the detection results to comfirm app behaviors.

\begin{figure}
\begin{minipage}[t]{0.47\linewidth}
\centering
\includegraphics[width=1.55in]{./picture/045.png}
\caption{Target state selector.}
\label{fig:side:a}
\end{minipage}%
\begin{minipage}[t]{0.47\linewidth}
\centering
\includegraphics[width=1.8in]{./picture/047.png}
\caption{State model displayer.}
\label{fig:side:b}
\end{minipage}
\label{fig:side}
\end{figure}

For demonstratation, We use the tool to reproduce the java.io.FileNotFoundException exception recorded by the detector. On the webpage, We can find out the corresponding snapshot number is 6, as is shown in Fig.~\ref{fig:side:a}. Enter 6 in the input field below the graph and click \emph{send}.

The testing program successfully search the shortest path to the profile page, as is shown in Fig.~\ref{fig:side:b}, and start exploring again. Once the testing program click on \emph{Take Picture} or \emph{Select from other}, the exception repeated again.


\message{ !name(Usage_scenarios.tex) !offset(-174) }


==> section/background.tex <==
\subsection{Android Apps}

\subsection{Model-based App Testing}
Model-based testing is an approach for software testing orchestrated around a model of the software under test. The model is an abstract representation of the software behavior. Android apps are event-driven programs,  where the app logics are executed given specific events, such as tapping on the screen, scrolling, and changing network status.




and is used to construct a suit of test cases to test the app. In general, the generated test cases should meet two requirements. On one hand, the coverage reached by the test cases should be as high as possible. On the other hand, the number of the test cases and the size of each test case should be small enough to make the test execution efficiently.

Android apps are event-driven programs, where the app logics are executed given specific events, such as tapping on the screen, scrolling, and changing network status. Therefore, the model of Android app under test is usually abstracted as a finite state machine:$$FSM=<STATE,EVENT,\delta,K,Q>$$
$STATE=\{s_i\}$ is a set of app state, where $s_i$ is represented by runtime information that can distinguish app states, such as program variables, UI, and system stack.
$EVENT=\{e_i\}$ is a set of events that can trigger app state transfer, where $e_i\in TYPE \times VALUE$ is the information that can characterize an event, including event type (tap, type, ect.) and event values (the view which users tap on, the value which users type in, etc.).
The transfer of app states is defined as a mapping function $\delta:STATE\times EVENT\rightarrow STATE, \delta(s_i,e)=s_j$, where $s_i,s_j\in STATE, e\in EVENT$, meaning that given the current state $s_i$ and an event $e$, the app can transfer to state $s_j$.
$K\subset STATE$ is the set of start states. $Q\subset STATE$ is the set of end states.

Given the above definition, a test case generated by the model can be defined as a set of app state transfers $<s_i,s_j>^n$ triggered by events $e_1,e_2,\dots,e_n$, where $e_1\in K$, $e_n\in Q$, and $n$ is the length of the generated test case.


==> section/evaluation.tex <==
To assess the efficiency and advantage of our model-based technique, we conduct two experiments to address the following two questions: first, whether our tool is superior than other automated testing tools.  Second, whether the tool can be applied to highly sophisticated business applications.

For the first question, in order to be comparable, we use a common set of mobile app benchmarks collected by [] and concerned two criteria while evaluating the selected tools.
 
1. Effectiveness of the automated testing tools. The effectiveness is defined that the input generated by tools should be able to trigger corresponding codes of tested application. A good testing tool should ideally cover as much behavior as possible.  We use code coverage to represent the effectiveness of tools.
2. feasibility of the automated testing tools. while effectiveness is the major concern when it comes to select the most adequate automated testing tool, the average time the tool consumes during testing has a great impact on its feasibility. We use time-coverage curve to quantify the extent of feasibility.
 
while testing a common set of applications is necessary for comparison, the fact that many of the tools used for comparison is no longer maintained greatly limits the range of optional applications. While Android platforms have greatly evolved in the last few years and the complexity of business owned application is rapidly increasing, it's vital to assess the performance and robutness of automated testing tools on modern business applications in order to cater for the high industrial demands. We selected ten applications on the google play top charts and used the same two criteria while evaluating the selected applications.
 
we now proceed to presenting the experiment setup and measurement procedures.
(1) Setup and Tools
Experiment 1:
In order to be comparable, we ran our tool on the publicly available Ubuntu 14.04 virtual machines, which is integrated with [] tools and benchmark applications thus guarantee a united testing environment. Each virtual machine was configured with 2 cores and 6GB RAM. The android emulator inside the virtual machine was configured to use 4GB RAM and each tool was allowed to run for 1 hour on each benchmark application. We chose Android SDK version 19(KitKat) to evaluate our tool based on the compatibility of most benchmark applications. To avoid unexpected side-effects between tools and application, the emulator is destroyed after finishing each run. To enhance the reliability of results, we repeated running each application for {} times.
 
Experiment 2:
We randomly select ten Applications on the Google play top charts as subjects to evaluate usability of tools on highly complicated bussiness applicaions. Due to the higher complexity of event logic and richer graphical effects of the business applications, we chose Genymotion, an optimized android emulator to perform the task. The emulator running in the physical machine was configured to 4GB RAM and each tool was allowed to run for 1 hour on each business applications. The Android SDK (version 19 KitKat) is set to be the same as experiment 1 and the emulator is destroyed after finishing each run. We repeated running each application for {} times. Because 7 applications require log in to access more information, we also sign up corresponding accounts and sign in before each run.

(2) Measuring coverage
For experiment 1, we selected Emma to measure code coverage of each tool and used benchmark applications which already been instrumented with emma on the virtual machine as subjects. To each benchmark, we use the same broadcast receiver solution mentioned in {} to save intermediate coverage results to the disk. The interval of intermediate coverage data storage is set to be 10 seconds. We parsed the HTML reports generated by emma to extract class, method, block and line coverage information. We also developed a tool to dynamically merge coverage data and display time-coverage curve.
 
For experiment 2, though the origin code of business applications is not available, which makes it impossible to implement applications with emma, we can still extract activities reached during execution using logcat utility provided by Android Debug Bridge(adb) tool from the Android SDK. The logcat filter is set to extract current testing application's displayed activity information. Android OS also provides an Application Manager(am) utility with method profiling options, which generate a trace files on runtime. The interval of profile start and stop is set to be 10 seconds and We parsed the generated trace files dynamically to extract the unique method reached during execution.



==> section/motivation.tex <==
In this section, we present a mitivating example to illustrate how can the previous approaches build the model and how to explore the app based on the model.
1. A motivating example



2. Research Question:
(1) State Identification:
As is discussed before, the fundamental task for model extraction is to identify a state precisely. Only consider the UI structure will bring state space explosion, and only consider activity will lose a lot of different states. Therefore, a novel state identification rule should be designed carefully to strike a balance between accuracy and compactness.
(2) app exploration:
Another question for model extraction is to build the model automatically and efficiently. To this end, the standard depth first search(DFS) crawling algorithm is utilized by various works. However, a major challenge for this DFS method is to implement backtrack step, i.e., returing to the previous state correctly and continuing crawling the undo event list in this state. However, as the android platform does not provide a explicit way to go back to the sprcific state, most of the work resort to frequent restart for backtracking, which is a tremendous waste for performance and efficiency. Therefore, a more efficient crawling framework that can efficiently explre the app and build the model is in great demand.
